NEXT-EVAL: Next Evaluation of Traditional and LLM Web Data Record Extraction

Effective evaluation of web data record extraction methods is crucial, yet hampered by static, domain-specific benchmarks and opaque scoring practices. This makes fair comparison between traditional algorithmic techniques, which rely on structural heuristics, and Large Language Model (LLM)-based approaches, offering zero-shot extraction across diverse layouts, particularly challenging. To overcome these limitations, we introduce a concrete evaluation framework. Our framework systematically generates evaluation datasets from arbitrary MHTML snapshots, annotates XPath-based supervision labels, and employs structure-aware metrics for consistent scoring, specifically preventing text hallucination and allowing only for the assessment of positional hallucination. It also incorporates preprocessing strategies to optimize input for LLMs while preserving DOM semantics: HTML slimming, Hierarchical JSON, and Flat JSON. Additionally, we created a publicly available synthetic dataset by transforming DOM structures and modifying content. We benchmark deterministic heuristic algorithms and off-the-shelf LLMs across these multiple input formats. Our benchmarking shows that Flat JSON input enables LLMs to achieve superior extraction accuracy (F1 score of 0.9567) and minimal hallucination compared to other input formats like Slimmed HTML and Hierarchical JSON. We establish a standardized foundation for rigorous benchmarking, paving the way for the next principled advancements in web data record extraction.

==> neurips/abstract.tex <==
Effective evaluation of web data record extraction methods is crucial, yet hampered by static, domain-specific benchmarks and opaque scoring practices. This makes fair comparison between traditional algorithmic techniques, which rely on structural heuristics, and Large Language Model (LLM)-based approaches, offering zero-shot extraction across diverse layouts, particularly challenging. To overcome these limitations, we introduce a concrete evaluation framework. Our framework systematically generates evaluation datasets from arbitrary MHTML snapshots, annotates XPath-based supervision labels, and employs structure-aware metrics for consistent scoring, specifically preventing text hallucination and allowing only for the assessment of positional hallucination. It also incorporates preprocessing strategies to optimize input for LLMs while preserving DOM semantics: HTML slimming, Hierarchical JSON, and Flat JSON. Additionally, we created a publicly available synthetic dataset by transforming DOM structures and modifying content. We benchmark deterministic heuristic algorithms and off-the-shelf LLMs across these multiple input formats. Our benchmarking shows that Flat JSON input enables LLMs to achieve superior extraction accuracy (F1 score of 0.9567) and minimal hallucination compared to other input formats like Slimmed HTML and Hierarchical JSON. We establish a standardized foundation for rigorous benchmarking, paving the way for the next principled advancements in web data record extraction.

==> neurips/experiment/dataset.tex <==
Our evaluation dataset consists of 164 real-world web pages, collectively containing over 12,278 annotated data records. Each page was selected from a diverse set of domains, including commerce, media, government, and social platforms. Pages were chosen based on their high popularity and rich presence of repeated content structures such as product listings, tables, article feeds, or ranked items. All pages were saved in MHTML format to preserve layout and interactive elements.

The dataset spans a wide range of domains: approximately 63 pages belong to \textit{e-commerce and shopping} platforms, 20 pages to \textit{entertainment and sports} sites, 15 to \textit{finance and investing}, 10 to \textit{news and media}, and 10 to \textit{education and research} portals. Additionally, there are pages from \textit{technology and development} (7), \textit{travel and hospitality} (7), \textit{real estate} (8), \textit{jobs and careers} (6), \textit{health and wellness} (6), \textit{coupons and deals} (6), \textit{government and public data} (5), \textit{social and community} (5), and \textit{food and dining} (4), ensuring structural diversity.

Each page contains a varying number of data records, ranging from a handful (e.g., 3) to over nine hundred (e.g., 913 for a site like Indeed.com). This distribution captures a broad spectrum of extraction scenarios—from simple, templated layouts to deeply nested or sparse structures. This dataset serves as a realistic and challenging benchmark for evaluating both traditional and LLM-based web data record extractors.

==> neurips/experiment/experiment.tex <==
\subsection{Implementation Details}
\input{experiment/setup.tex}

\subsection{Dataset}
\label{sec:exp-dataset}
\input{experiment/dataset.tex}

\subsection{Results}
\input{experiment/results.tex}

==> neurips/experiment/results.tex <==
\begin{table}[h]
    \centering
    \caption{Average token counts for different input types.}
    \label{tab:token_counts}
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{lccc}
    \toprule
    & Slimmed HTML & Hierarchical JSON & Flat JSON \\
    \midrule
    Average Tokens & 86,084 & 34,107 & 116,698 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}[h]
    \centering
    \caption{Extraction performance of non-visual methods.}
    \label{tab:results_nonvisual}
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{llcccc}
    \toprule
    Method & Input Type & Precision & Recall & F1 Score & Hallucination Rate\\
    \midrule
    MDR \citep{mdr} & Full / Slimmed HTML & 0.0746 & 0.1593 & 0.0830 & \textbf{0.0000}\\
    \midrule
    Gemini-2.5-pro-preview-03-25 & Slimmed HTML & 0.1217  & 0.0969 & 0.1014 & 0.9146\\
                                 & Hierarchical JSON &0.4932 &  0.3802 & 0.4048  & 0.5976\\
                                 & Flat JSON & \textbf{0.9939} & \textbf{0.9392} & \textbf{0.9567}  & 0.0305 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

The experimental results highlight the significant impact of input representation on the performance of LLM-based web data extractors. \Cref{tab:token_counts} details the average token counts for the different input types. Hierarchical JSON is the most token-efficient, with an average of 34,107 tokens. Slimmed HTML follows with 86,084 tokens, while Flat JSON is the least token-efficient, requiring an average of 116,698 tokens. This data underscores the varying textual complexities of each representation.

\Cref{tab:results_nonvisual} presents the extraction performance for non-visual methods. Gemini-2.5-pro-preview, when provided with Flat JSON input, achieves the highest performance with a precision of 0.9939, recall of 0.9392, and an F1 score of \textbf{0.9567}. This strong performance is attributed to the unambiguous localization of fields offered by Flat JSON (as described in \Cref{subsec:apiOpt}) and a remarkably low hallucination rate of 0.0305. The reduced hallucination stems from the relative ease with which the LLM can infer structural information and XPath-like paths from JSON compared to HTML. However, it is noted that for URLs with deep hierarchical structures, hallucination can still occur in approximately 3\% of cases with Flat JSON.

When using Hierarchical JSON, which mirrors the DOM tree structure to aid the model in understanding parent-child relationships (\Cref{subsec:apiOpt}), Gemini-2.5-pro-preview achieves a precision of 0.4932, recall of 0.3802, and an F1 score of 0.4048, with a hallucination rate of 0.5976. While not as performant as Flat JSON, this input type still offers a significant reduction in hallucination compared to HTML-based inputs, as the JSON format provides a clearer structural representation for the LLM.

In contrast, Gemini-2.5-pro-preview's performance with Slimmed HTML input (0.1217 P, 0.0969 R, 0.1014 F1) is considerably lower. This is largely due to a very high hallucination rate of 0.9146. Directly parsing complex web structures and inferring XPaths from HTML, even a compressed version like Slimmed HTML (see \Cref{subsec:apiOpt}), proves challenging for the LLM, leading to frequent hallucinations of invalid elements.

The traditional baseline, MDR, operating on Full or Slimmed HTML, shows a precision of 0.0746, recall of 0.1593, and an F1 score of 0.0830. Notably, MDR exhibits no hallucination (\textbf{0.0000}) due to its intrinsic design. However, its low precision and recall stem from its tendency to extract all potential data records, thereby reducing precision, and its inability to consistently identify and extract exact data records or all their similar counterparts comprehensively, which lowers recall. These characteristics suggest that MDR's output may require significant additional post-processing to refine the extracted data.

These findings collectively underscore the critical role of input representation and careful prompt engineering in unlocking the full potential of LLMs for complex tasks such as web data record extraction. The choice of input format directly influences not only the model's accuracy but also its propensity for hallucination, with structured formats like JSON offering more reliable pathways for information retrieval.

Furthermore, to facilitate broader research and ensure data privacy, we developed a synthetic dataset. This dataset was constructed by systematically transforming the DOM structures and modifying the textual content of the original web pages. The creation of this synthetic dataset enables the public dissemination of a diverse and challenging benchmark for web data extraction tasks. The detailed experimental results on this synthetic dataset are included in the supplementary material, and the dataset itself will be made publicly available. 

==> neurips/experiment/setup.tex <==
We evaluate a traditional web data record extraction method—MDR—as well as a modern LLM-based extractor. For the latter, we leveraged the Gemini-2.5-pro-preview-03-25 model \citep{team2023gemini}, accessed via its API, using the default temperature setting of 1.0. This specific model was selected due to its extensive input token allowance, which enabled us to perform experiments on the largest possible number of websites from our dataset. Each method is tested on a diverse dataset of real-world web pages; a detailed description of this dataset is provided in \Cref{sec:exp-dataset}. Explicit site list is available in the supplementary material. Ground-truth annotations are provided as sets of XPath expressions identifying repeated data records.

We do not include DEPTA and NET in our evaluation, as they rely on visual layout cues (e.g., rendered bounding boxes), which are not available without a rendering pipeline. In contrast, MDR operates purely on the DOM structure and is thus directly comparable to our LLM-based approach.

For the LLM-based approach, we design HTML prompts tailored for Gemini-2.5-pro-preview-03-25 to balance performance and token efficiency. We considered an approach using (a) \emph{Full HTML}, which includes all original attributes such as class names, IDs, and precise positional information. However, this method presents challenges for a fair comparison, as these attributes provide cues not available to other preprocessing techniques. Furthermore, Full HTML is substantially larger, often more than ten times the size of \emph{Slimmed HTML}, frequently exceeding input token limits and thereby restricting the number of websites on which experiments can be conducted. Consequently, we excluded Full HTML from our primary evaluation. Instead, we evaluate three distinct preprocessing strategies for constructing the prompts: (b) \emph{Slimmed HTML}, where verbose attributes are removed while preserving DOM structure; (c) \emph{Hierarchical JSON}, which reflects the hierarchical structure of the original DOM in a JSON-like nested form; and (d) \emph{Flat JSON}, which flattens the HTML into a key-value mapping from XPath to textual content. These variants allow for flexible trade-offs between structural fidelity and token compactness.

Since the exact token count cannot be determined before submission, we report the final token usage based on the serialized prompts actually sent to the LLM. Details of our prompting strategies and input formats are described in \Cref{subsec:apiOpt}.

==> neurips/figures/htmlInputEx.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
\begin{lstlisting}[language=html]
<html>
  <body>
    <ul class="product-list">
      <li class="item"><span class="name">Sample Product</span></li>
      <li class="item"><span class="price">$999.00</span></li>
    </ul>
  </body>
</html>
\end{lstlisting}
    \subcaption{Original HTML}\label{fig:orig_html}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
\begin{lstlisting}[language=html]
<html>
  <body>
    <ul>
      <li><span>Sample Product</span></li>
      <li><span>$999.00</span></li>
    </ul>
  </body>
</html>
\end{lstlisting}
    \subcaption{Slimmed HTML (attributes removed)}\label{fig:slim_html}
  \end{subfigure}

  \vspace{0.8em} % vertical spacing between rows

  \begin{subfigure}[b]{0.45\linewidth}
    \centering
\begin{lstlisting}[language=java]
{
  "html": {
    "body": {
      "ul": {
        "li[1]": { "span": "Sample Product" },
        "li[2]": { "span": "$999.00" }
      }
    }
  }
}
\end{lstlisting}
    \subcaption{Hierarchical JSON (Nested text map)}\label{fig:hier_map}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
\begin{lstlisting}[language=java]
{
  "/html/body/ul/li[1]/span": "Sample Product",
  "/html/body/ul/li[2]/span": "$999.00"
}
\end{lstlisting}
    \subcaption{Flat JSON (text map)}\label{fig:flat_xpath}
  \end{subfigure}

  \caption{
  Input representations for LLM-based data extraction, corresponding to types evaluated in \Cref{tab:token_counts,tab:results_nonvisual}.
  (a)~Original HTML with attributes often treated as noise.
  (b)~Slimmed HTML, created by pruning attributes from the original HTML.
  (c)~Hierarchical JSON, a token-efficient, nested representation of the DOM structure.
  (d)~Flat JSON, mapping XPaths to their corresponding text content for precise localization.
  }
  \label{fig:htmlInputEx}
\end{figure}


==> neurips/introduction.tex <==
Web is a vast and dynamic source of structured and semi-structured information. Much of this information, found in natural language descriptions, tables, and repetitive patterns, is amenable to extraction and analysis. Extracting structured data records—repeating content elements from web pages—has significant utility across many practical applications \citep{webtables, websurvey, briefwebsurvey, extractStruct, hierarchicalWrapper}. For example, office workers frequently need to collect structured information, such as product listings, company directories, and contact tables from websites, and store it in spreadsheets or internal databases. Automating this process can lead to substantial productivity gains.

Traditional web data record extraction has primarily relied on structural heuristics that analyze HTML trees to detect repetitive patterns \citep{buttler, iepad, mdr, depta, net}. While these methods have achieved some success, their efficacy is often hampered by a reliance on rigid structural assumptions. This limits their ability to generalize across diverse and dynamic web layouts. Furthermore, these methods largely overlook textual semantics, leading to instability when visual or structural cues alone are insufficient.

In contrast, Large Language Models (LLMs) have recently shown remarkable capabilities in natural language understanding, reasoning, and information extraction \citep{llm1,largellm,gpt3,bert}. These models offer a promising new paradigm for web data record extraction, potentially working alongside or enhancing traditional heuristic methods \citep{net, depta, mdr}. However, deploying LLMs in real-world scenarios presents challenges: (i) fine-tuning LLMs is resource-intensive, and (ii) LLMs inherently grapple with issues such as hallucination and a lack of transparency in their decision-making processes.

Moreover, the evaluation of LLM-based extraction methods is hindered by the absence of standardized, publicly available datasets. Existing datasets are often domain-specific and restricted by terms of service or `robots.txt' directives, limiting their utility for benchmarking. This situation highlights the critical need for a general-purpose dataset and a concrete evaluation framework to assess and compare the efficacy of traditional and LLM-based extraction methods.

In this work, we introduce a practical evaluation framework for comparing traditional algorithms and LLMs on the task of web data record extraction. Our contributions are as follows:

\begin{itemize}
\item We propose a reproducible framework that constructs evaluation datasets from arbitrary MHTML web snapshots. Our framework provides XPath-based structured outputs and the corresponding URLs for the datasets we evaluated.
\item We establish a concrete scoring framework to evaluate both heuristic algorithms (e.g., XPath wrappers, partial tree alignment) and LLM-based methods. Our protocol thoroughly prevents distortions from hallucination and supports partial credit through structure-aware matching.
\item We explore how to optimize raw HTML input for LLM-based methods by introducing preprocessing strategies that reduce token length while preserving the semantic and structural integrity of the page. These strategies include HTML slimming, and converting HTML into structured representations like Hierarchical JSON and Flat JSON. Our results demonstrate that these formats significantly influence extraction performance and hallucination rates.
\item We created a publicly available synthetic dataset by transforming DOM structures and modifying content from original web pages.
\end{itemize}

This work lays a foundational cornerstone for future research in web record extraction, particularly for developing text-aware and HTML-friendly methods in the era of LLMs.


==> neurips/method/apiOpt.tex <==
To enable a rigorous evaluation of LLM extractors on web pages, we propose a preprocessing framework that simultaneously (i) compresses raw HTML to stay within the LLM token budget, and (ii) preserves the full DOM hierarchy so that ground-truth labels can still be expressed as absolute XPaths.

One of the key constraints when using LLM APIs is the token limit per request. To address this, we applied several preprocessing techniques to reduce input size without sacrificing structural semantics. Unlike plain text or Markdown, which may be more compact, these formats do not retain absolute DOM positions necessary for XPath supervision. Therefore, we maintain the original HTML structure while removing unnecessary attributes—such as \texttt{class}, \texttt{id}, and \texttt{style}—that are often verbose and semantically redundant. This results in a lightweight yet structurally faithful HTML tree. For example, we convert \Cref{fig:orig_html} into \Cref{fig:slim_html}.

In addition to HTML-based inputs, we explored JSON-based formats to guide the model more explicitly. First, we construct a \emph{Hierarchical JSON} (\Cref{fig:hier_map}), which mirrors the DOM tree hierarchy in JSON form. Although slightly more verbose in tokens than flattened formats, this hierarchical structure helps the model understand parent-child relationships, reducing the risk of hallucinating invalid elements.

Second, we construct a \emph{Flat JSON} (\Cref{fig:flat_xpath}), where each key is an absolute XPath and the value is the corresponding textual content. While this format discards hierarchy from the nested structure, it provides unambiguous localization of each field, ensuring token-level precision during decoding.

Ultimately, the framework lets us evaluate extractors purely on positional accuracy: a model's output is valid only if the text content of the predicted XPath exists in the cleaned DOM. Since every model output paths are drawn from the cleaned DOM, the model cannot hallucinate elements that do not exist. 

\lstset{
  basicstyle=\ttfamily\small,
  columns=fullflexible,
  frame=single,
  breaklines=true
}
\input{figures/htmlInputEx}


==> neurips/method/dataset.tex <==
To support fair and rigorous evaluation, we construct a large and general-purpose dataset. It encompasses a wide variety of web domains, significantly broadening the scope beyond prior datasets like PLAte~\citep{plate} which were often restricted to specific categories such as shopping pages. Our dataset is designed to capture repetitive structures and a variety of DOM structures across this diverse range, including many non-product-centric pages.

Each web page is stored in MHTML format to preserve all layout and interactive elements. From each page, we annotate the main repeated data records using XPath expressions. These XPaths serve as ground-truth labels for evaluation.

To identify data records, we first leverage large language models (LLMs) to automatically annotate candidate repetitive blocks in each page. Human annotators then review and refine these suggestions to ensure high-quality labels. This semi-automatic process balances scalability and accuracy.

Using XPath as the supervision format enables deterministic and verifiable evaluation grounded in the DOM structure. Unlike free-text descriptions, XPath annotations constrain model predictions to concrete, observable elements on the page. This prevents hallucinations where LLMs infer data records from unrelated textual context by requiring that every predicted record maps to an exact DOM node. As LLMs may generate plausible-looking but structurally invalid groupings, XPath-based evaluation ensures alignment with the actual HTML hierarchy.

==> neurips/method/definition.tex <==
We formalize web data record extraction as the task of identifying repeated sets of semantically related elements in a web page's DOM tree. As defined in \Cref{sec:prelim}, each data record corresponds to a set of XPath expressions whose associated DOM nodes together describe a single coherent entity (e.g., a product or listing).

Given an HTML document, let \( \mathcal{X} \) denote the set of all XPath expressions referencing non-trivial text nodes. The goal is to segment this set into \( \mathcal{P} = \{P_1, \dots, P_M\} \), where each \( P_i \subseteq \mathcal{X} \) forms a data record.

Unlike traditional attribute extraction, we treat the internal structure of a record as a black box and focus solely on discovering consistent repeating record-level groupings. These groups may appear as contiguous siblings in the DOM or may be non-contiguous and nested under different parent elements.

This task can be viewed as the inverse of web page templating: rather than generating HTML from structured data, we recover the structured data (as XPath sets) from rendered HTML. This inversion is particularly challenging in real-world pages, where markup irregularities, dynamic content, and layout noise are common.

In our approach, we leverage LLM APIs to perform this extraction via carefully designed HTML prompts. The details of our prompting strategies and API usage are presented in \Cref{subsec:apiOpt}.

==> neurips/method/evaluation.tex <==
We evaluate data record extraction methods by comparing predicted record sets against human-annotated ground truth. Each data record is represented as a set of XPath expressions, and the comparison is performed at the record level using a matching-based evaluation framework.

Let \( \mathcal{P} = \{P_1, \dots, P_M\} \) denote the set of predicted records, and \( \mathcal{G} = \{G_1, \dots, G_N\} \) the set of ground-truth records, where each \( P_i, G_j \subset \mathcal{P} \) is a set of XPath expressions. For each pair \( (P_i, G_j) \), we define an \emph{overlap score} as the Jaccard similarity between the two sets:
\begin{align}
\mathrm{Overlap}(P_i, G_j) = \frac{|P_i \cap G_j|}{|P_i \cup G_j|}
\end{align}

To evaluate the quality of extraction, we compute an optimal one-to-one matching \( \mathcal{M} \subseteq \mathcal{P} \times \mathcal{G} \) that maximizes the total overlap across matched pairs. This is solved using the Hungarian algorithm. Based on the optimal alignment \( \mathcal{M} \), we define precision and recall as:
\begin{align}
  \mathrm{Precision} &= \frac{1}{|\mathcal{P}|} \max_{\mathcal{M} \subseteq \mathcal{P} \times \mathcal{G}} \sum_{(P_i, G_j) \in \mathcal{M}} \mathrm{Overlap}(P_i, G_j) \\
  \mathrm{Recall} &= \frac{1}{|\mathcal{G}|} \max_{\mathcal{M} \subseteq \mathcal{P} \times \mathcal{G}} \sum_{(P_i, G_j) \in \mathcal{M}} \mathrm{Overlap}(P_i, G_j)
\end{align}

The final F1 score is computed as the harmonic mean of precision and recall:
\begin{align}
\mathrm{F1} = \frac{2 \cdot \mathrm{Precision} \cdot \mathrm{Recall}}{\mathrm{Precision} + \mathrm{Recall}}
\end{align}

In addition to these metrics, we also assess the Hallucination Rate (HR). For each web page (URL) in our test set, a hallucination event is considered to have occurred (value of 1) if the model predicts at least one empty record (i.e., a record containing no corresponding XPaths); otherwise, it is 0. The Hallucination Rate is then the average of these binary hallucination event indicators across all processed URLs for which predictions are available. A lower HR is preferable, indicating that the model is less prone to generating empty, and thus unusable, records.

This formulation allows for partial credit when records are only partially correct (e.g., missing fields or over-segmentation), and is robust to variations in record granularity or representation (e.g., nested vs. flat XPath sets). Unlike token-level or text-based matching, this metric directly reflects correctness at the structural level, which is essential for applications requiring XPath-based or DOM-aligned outputs.


==> neurips/method/method.tex <==
\subsection{Problem Setting}
\input{method/definition.tex}

\subsection{Dataset Construction}
\input{method/dataset.tex}

\subsection{Preprocessing for LLMs}
\label{subsec:apiOpt}
\input{method/apiOpt.tex}

\subsection{Evaluation Framework}
\input{method/evaluation.tex}

==> neurips/prelim.tex <==
To formally represent and extract structured content from HTML pages, we rely on XPath expressions. An XPath \( x \in \mathcal{X} \) is a path-like expression that identifies a unique node in the DOM (Document Object Model) tree. XPath expressions encode the structural position of elements in the HTML tree, and the relationships among them reflect the hierarchical layout of web content.

Structured content on the web—such as product listings, hotel entries, or user profiles—is typically composed of repeated logical units called \emph{data records}. A data record refers to a group of semantically related elements that together describe a single entity.

\begin{definition}[Data Record]
Let \( \mathcal{X} \) be the set of XPath expressions in a document. A data record \( X_i \subseteq \mathcal{X} \) is defined as a finite set of XPath expressions whose corresponding DOM nodes contain non-trivial textual content (i.e., not empty or purely whitespace) and collectively represent a coherent, repeated unit on the page.
\end{definition}

This set-based definition naturally accommodates both simple and complex structures—whether the relevant elements are grouped under one parent node or distributed across different DOM branches. It also allows for nested or non-contiguous layouts to be expressed without relying on a single subtree.

\textbf{Example.} Consider the following HTML snippet:

\lstset{
  basicstyle=\ttfamily\small,
  columns=fullflexible,
  frame=single,
  breaklines=true
}
\begin{lstlisting}[language=html] 
<div class="product">
  <div class="image">
    <img src="a.jpg"/>
    <span class="caption">A beautiful image</span>
  </div>
  <div class="info">
    <span class="name">Camera</span>
    <span class="price">$399</span>
  </div>
</div>
\end{lstlisting}

The corresponding data record can be represented as:

\[
X_1 = \left\{
\texttt{/div[1]/div[1]/span[1]}, 
\texttt{/div[1]/div[2]/span[1]}, 
\texttt{/div[1]/div[2]/span[2]}
\right\}
\]

This approach captures all relevant fields of the product as a set of XPath references. In more complex settings—such as when parts of a record appear in different sections of the DOM—this model remains consistent and expressive. We discuss such cases, including nested and non-contiguous records, in the supplementary material.


==> neurips/preliminary/nested.tex <==
\paragraph{Nested Data Records.}
More complex objects may include nested sub-records. For example, a hotel might contain a set of user reviews, where each review is itself a repeated substructure. Below is an example with two such nested records:

\vspace{0.5em}
\noindent\textbf{Nested Record Example:}

\begin{minipage}{0.48\columnwidth}
\begin{adjustbox}{width=\columnwidth}
\begin{lstlisting}[language=HTML, basicstyle=\ttfamily\small]
<div class="hotel">
  <span class="hotel-name">Hotel A</span>
  <div class="review">
    <span class="author">User1</span>
    <span class="text">Great stay!</span>
  </div>
  <div class="review">
    <span class="author">User2</span>
    <span class="text">Okay experience.</span>
  </div>
</div>
\end{lstlisting}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{0.48\columnwidth}
\small
\[
\begin{aligned}
P_1 = \{ &\texttt{/div[1]/span}, \\
         &\texttt{/div[1]/div[1]/span[1]}, \\
         &\texttt{/div[1]/div[1]/span[2]} \} \\
\\
P_2 = \{ &\texttt{/div[1]/span}, \\
         &\texttt{/div[1]/div[2]/span[1]}, \\
         &\texttt{/div[1]/div[2]/span[2]} \}
\end{aligned}
\]
\end{minipage}

\vspace{1em}
This hierarchical layout is typical in web applications that embed comments, nested listings, or reviews. Algorithms such as DEPTA and AMBER~\citep{amber} address these cases by leveraging partial alignment between repeated structures, as well as semantic annotations.


==> neurips/preliminary/noncontiguous.tex <==
\paragraph{Non-contiguous Data Records.}
In more complex web layouts, object descriptions may be interleaved across disjoint DOM segments. A common case appears in grid-based or tabular designs where different fields of the same object are separated. Consider the following two-row layout:

\vspace{0.5em}
\noindent\textbf{Non-contiguous Record Example:}

\begin{minipage}{0.48\columnwidth}
\begin{adjustbox}{width=\columnwidth}
\begin{lstlisting}[language=HTML, basicstyle=\ttfamily\small]
<tr>
  <td class="name">Camera</td>
  <td class="name">Laptop</td>
</tr>
<tr>
  <td class="price">$399</td>
  <td class="price">$899</td>
</tr>
\end{lstlisting}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{0.48\columnwidth}
\small
\[
\begin{aligned}
P_1 = \{ &\texttt{/tr[1]/td[1]}, \\
         &\texttt{/tr[2]/td[1]} \} \\
\\
P_2 = \{ &\texttt{/tr[1]/td[2]}, \\
         &\texttt{/tr[2]/td[2]} \}
\end{aligned}
\]
\end{minipage}

\vspace{1em}
Although each product’s name and price are visually aligned, their DOM paths are separated. DEPTA~\citep{depta} proposes aligning corresponding child nodes across rows to reconstruct full records. This form of non-contiguity challenges traditional subtree-based extraction methods and motivates structural merging based on positional correspondence.


==> neurips/preliminary/partialOrder.tex <==
\begin{definition}[XPath Partial Order]
Let \( \mathcal{P} \) be the set of XPath expressions in an HTML page. We define a partial order \( \succeq \) over \( \mathcal{P} \) such that for any \( p_i, p_j \in \mathcal{P} \), we say \( p_i \succeq p_j \) if and only if \( p_i \) is an ancestor of \( p_j \) in the DOM tree. That is, \( p_j \) can be formed by appending additional tag steps to \( p_i \).

\textbf{Example:}
\[
\begin{aligned}
p_i &= \texttt{/html/body/div[2]/span[1]} \\
p_j &= \texttt{/html/body/div[2]/span[1]/div[5]/div[2]}
\end{aligned}
\]
Since \( p_j \) extends \( p_i \), we have \( p_i \succeq p_j \). This structure allows us to reason about hierarchical containment and record grouping within the document.
\end{definition}

==> neurips/related/benchmark.tex <==
Benchmark datasets are crucial for evaluating and comparing information extraction methods. PLAtE \citep{plate} is a large-scale dataset designed for list page web extraction, focusing on product segmentation and attribute extraction. While PLAtE provides valuable resources for specific domains, its static nature and domain-specific focus limit its applicability across diverse web contexts.

AMBER \citep{amber} introduces a semi-automatic extraction system targeting multi-attribute objects from deep web pages, such as real estate listings. Although its rule-based annotations offer high precision, it lacks publicly available datasets and generalizability across web domains. The dataset used in AMBER—real estate and car listings—is extensive but domain-limited and not openly accessible, restricting its utility for reproducible benchmarks.

The Klarna Product Page Dataset \citep{klarna} provides a high-quality resource for training and evaluating web element nomination methods. It includes detailed annotations for product pages using graph-based and LLM-based labeling strategies. However, its scope is confined to e-commerce, and the data cannot be redistributed due to licensing constraints. While it supports fine-grained element labeling, it does not directly support data record segmentation or structural evaluation using tree-based supervision.

Multi-Record Web Page Extraction \citep{multiRecord} focuses on news websites and introduces methods to extract multiple records from a single page. While it demonstrates the value of domain-specific modeling (e.g., headlines, summaries), it does not provide a publicly reusable dataset or a unified evaluation protocol, and relies on heuristics that are tightly coupled with the news domain structure.

These efforts highlight the growing need for evaluation datasets that are (i) publicly available, (ii) structurally diverse across domains, and (iii) compatible with both rule-based and LLM-based methods. Our work addresses this by introducing a framework and a benchmark dataset built from diverse MHTML web snapshots. Key contributions include human-refined XPath annotations for robust, DOM-grounded evaluation, and a scoring system that penalizes LLM hallucination. Furthermore, we developed a publicly available synthetic dataset to foster broader research.

==> neurips/related/llm.tex <==
The advent of LLMs has revolutionized information extraction tasks. Models like GPT-3.5 \citep{gpt35} and GPT-4 \citep{gpt4} have demonstrated remarkable capabilities in understanding and generating human-like text. Recent studies have explored the application of LLMs for extracting structured information from web pages. For instance, \citet{llmAttribute} investigated the zero-shot extraction and normalization of product attribute values using GPT models, achieving competitive performance without task-specific training data.

Another line of research focuses on enhancing the understanding of web page structures, for which specialized models like MarkupLM have been introduced. MarkupLM is a pre-trained model designed for document understanding tasks that utilize markup languages, such as HTML, where text and markup information are jointly pre-trained \citep{markUpLM}. This model incorporates additional embedding layers to capture the hierarchical structure of HTML documents, improving performance on tasks like information extraction from web pages.

==> neurips/related/related.tex <==
\subsection{Traditional Methods and Heuristic Approaches}

\input{related/traditional}

\subsection{Large Language Model–Based Approaches}

\input{related/llm}

\subsection{Benchmark Datasets and Evaluation Frameworks}

\input{related/benchmark}

==> neurips/related/traditional.tex <==
Early web data record extraction approaches relied on heuristic-based algorithms that exploited regularities in the HTML structure of web pages \citep{buttler, iepad, mdr, depta, net}. A representative example is the Mining Data Records (MDR) algorithm, which segments web pages into data regions by analyzing the DOM tree and detecting repeated sibling structures \citep{mdr}. MDR is effective when records are arranged contiguously in a clean and regular HTML layout. However, it struggles in scenarios where data records are non-contiguous—i.e., interleaved with unrelated elements or separated by visual gaps—because it assumes strict adjacency in the DOM.

To overcome these limitations, \citet{depta} proposed DEPTA (Data Extraction based on Partial Tree Alignment), which decouples segmentation and alignment. First, it identifies candidate data regions using structural and visual cues. Then, it performs partial tree alignment to recover repeated substructures, even when records are not adjacent in the HTML. This makes DEPTA more robust to noisy layouts and capable of handling non-contiguous record structures.

Building on this, NET incorporates visual features such as the rendered bounding boxes of elements to extract both flat and nested data records \citep{net}. By leveraging layout-based cues in addition to DOM structure, NET is better suited for complex templates and deeply nested hierarchies.

A more recent system, AMBER, introduces automatic supervision to reduce reliance on manually crafted rules \citep{amber}. It uses entity recognizers (e.g., for names, prices, dates) to label semantically meaningful parts of the page, and aligns these semantic hints with repeated DOM structures. This alignment improves extraction robustness on attribute-rich, template-based, and noisy web pages.


==> preliminary/nested.tex <==
\paragraph{Nested Data Records.}
More complex objects may include nested sub-records. For example, a hotel might contain a set of user reviews, where each review is itself a repeated substructure. Below is an example with two such nested records:

\vspace{0.5em}
\noindent\textbf{Nested Record Example:}

\begin{minipage}{0.48\columnwidth}
\begin{adjustbox}{width=\columnwidth}
\begin{lstlisting}[language=HTML, basicstyle=\ttfamily\small]
<div class="hotel">
  <span class="hotel-name">Hotel A</span>
  <div class="review">
    <span class="author">User1</span>
    <span class="text">Great stay!</span>
  </div>
  <div class="review">
    <span class="author">User2</span>
    <span class="text">Okay experience.</span>
  </div>
</div>
\end{lstlisting}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{0.48\columnwidth}
\small
\[
\begin{aligned}
P_1 = \{ &\texttt{/div[1]/span}, \\
         &\texttt{/div[1]/div[1]/span[1]}, \\
         &\texttt{/div[1]/div[1]/span[2]} \} \\
\\
P_2 = \{ &\texttt{/div[1]/span}, \\
         &\texttt{/div[1]/div[2]/span[1]}, \\
         &\texttt{/div[1]/div[2]/span[2]} \}
\end{aligned}
\]
\end{minipage}

\vspace{1em}
This hierarchical layout is typical in web applications that embed comments, nested listings, or reviews. Algorithms such as DEPTA and AMBER~\citep{amber} address these cases by leveraging partial alignment between repeated structures, as well as semantic annotations.


==> preliminary/noncontiguous.tex <==
\paragraph{Non-contiguous Data Records.}
In more complex web layouts, object descriptions may be interleaved across disjoint DOM segments. A common case appears in grid-based or tabular designs where different fields of the same object are separated. Consider the following two-row layout:

\vspace{0.5em}
\noindent\textbf{Non-contiguous Record Example:}

\begin{minipage}{0.48\columnwidth}
\begin{adjustbox}{width=\columnwidth}
\begin{lstlisting}[language=HTML, basicstyle=\ttfamily\small]
<tr>
  <td class="name">Camera</td>
  <td class="name">Laptop</td>
</tr>
<tr>
  <td class="price">$399</td>
  <td class="price">$899</td>
</tr>
\end{lstlisting}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{0.48\columnwidth}
\small
\[
\begin{aligned}
P_1 = \{ &\texttt{/tr[1]/td[1]}, \\
         &\texttt{/tr[2]/td[1]} \} \\
\\
P_2 = \{ &\texttt{/tr[1]/td[2]}, \\
         &\texttt{/tr[2]/td[2]} \}
\end{aligned}
\]
\end{minipage}

\vspace{1em}
Although each product’s name and price are visually aligned, their DOM paths are separated. DEPTA~\citep{depta} proposes aligning corresponding child nodes across rows to reconstruct full records. This form of non-contiguity challenges traditional subtree-based extraction methods and motivates structural merging based on positional correspondence.


==> preliminary/partialOrder.tex <==
\begin{definition}[XPath Partial Order]
Let \( \mathcal{P} \) be the set of XPath expressions in an HTML page. We define a partial order \( \succeq \) over \( \mathcal{P} \) such that for any \( p_i, p_j \in \mathcal{P} \), we say \( p_i \succeq p_j \) if and only if \( p_i \) is an ancestor of \( p_j \) in the DOM tree. That is, \( p_j \) can be formed by appending additional tag steps to \( p_i \).

\textbf{Example:}
\[
\begin{aligned}
p_i &= \texttt{/html/body/div[2]/span[1]} \\
p_j &= \texttt{/html/body/div[2]/span[1]/div[5]/div[2]}
\end{aligned}
\]
Since \( p_j \) extends \( p_i \), we have \( p_i \succeq p_j \). This structure allows us to reason about hierarchical containment and record grouping within the document.
\end{definition}
